The NIRSpec Wide GTO Survey

The Near-infrared Spectrograph (NIRSpec) on the James Webb Space Telescope is uniquely suited to studying galaxies in the distant Universe with its combination of multi-object capabilities and sensitivity over a large range in wavelength (0.6-5.3 microns). Here we present the NIRSpec Wide survey, part of the NIRSpec Instrument Science Team's Guaranteed Time Observations, using NIRSpec's microshutter array to obtain spectra of more than 3200 galaxies at $z>1$ at both low- and high-resolution ($R\approx100$ and 2700) for a total of 105 hours. With 31 pointings covering $\approx$320 arcmin$^2$ across the five CANDELS fields with exquisite ancillary photometry from the Hubble Space Telescope, the NIRSpec Wide survey represents a fast and efficient way of using JWST to probe galaxies in the early Universe. Pointing centers are determined to maximize the observability of the rarest, high-value sources. Subsequently, the microshutter configurations are optimized to observe the maximum number of "census" galaxies with a selection function based primarily on HST/F160W magnitude, photometric/slitless grism redshift, and predicted \ha\ flux tracing the bulk of the galaxy population at cosmic noon ($z_{\rm med}=2.0$). We present details on the survey strategy, the target selection, an outline of the motivating science cases, and discuss upcoming public data releases to the community.

==> table.tex <==

\longtab{\begin{longtable}{ccccccc}
 \caption{Wide targets in the AEGIS field, which will have spectra released as part of the initial data release (see Section \ref{sec:release}).  ``Other ID'' refers to IDs in the following catalogs: ``CANDELS,'' \citet{2017ApJS..229...32S}; ``ACS,'' \citet{2008ApJ...672..177L}; ``HSC,'' \citet{2019PASJ...71..114A}; ``EGS,'' \citet{2015ApJ...803...34B}. \label{tab:catalog}}\\
  Wide ID & 3D-HST ID & Other ID & RA  & Dec & F160W magnitude & Priority Class\\
  \hline
  \endhead
  \endfoot
2017000479&10045&CANDELS\_7846&215.19649&53.03309&24.34&7 \\ 
2017000560&10804&CANDELS\_8394&215.18492&53.02848&26.22&14 \\ 
2017000598&11135&CANDELS\_8654&215.19941&53.03987&24.91&10 \\ 
2017000687&11656&CANDELS\_9071&215.18571&53.03214&23.58&9 \\ 
2017000760&12233&CANDELS\_9506&215.18370&53.03346&25.67&7 \\ 
2017000795&12385&CANDELS\_9684&215.20399&53.04786&24.11&7 \\ 
2017000817&12636&CANDELS\_9844&215.18829&53.03757&22.45&14 \\ 
2017000840&&CANDELS\_9981&215.18574&53.03713&27.37&7 \\ 
2017000853&12967&CANDELS\_10067&215.19470&53.04400&25.71&7 \\ 
2017000883&13099&CANDELS\_10194&215.18562&53.03636&22.76&14 \\ 
2017000932&13410&CANDELS\_10466&215.17507&53.03150&24.02&10 \\ 
2017000971&13683&CANDELS\_10667&215.19771&53.04656&22.32&9 \\ 
2017001162&14976&CANDELS\_11752&215.16600&53.03140&22.62&14 \\ 
2017001248&15692&CANDELS\_12221&215.21347&53.06796&25.69&10 \\ 
2017001266&15807&CANDELS\_12328&215.17635&53.04239&25.32&7 \\ 
2017001277&15873&CANDELS\_12390&215.16387&53.03279&22.67&9 \\ 
2017001286&15986&CANDELS\_12428&215.17945&53.04523&25.43&7 \\ 
2017001325&16222&CANDELS\_12618&215.16802&53.03791&24.43&7 \\ 
2017001355&16423&CANDELS\_12764&215.16713&53.03861&25.96&15 \\ 
2017001371&16544&CANDELS\_12872&215.18252&53.04993&26.33&15 \\ 
2017001373&16582&CANDELS\_12894&215.21710&53.07433&26.81&15 \\ 
2017001397&16729&CANDELS\_13006&215.20236&53.06458&26.47&7 \\ 
2017001403&16634&CANDELS\_13036&215.19904&53.06156&23.87&9 \\ 
2017001431&16878&CANDELS\_13167&215.21702&53.07494&23.72&9 \\ 
2017001508&17355&CANDELS\_13528&215.16232&53.03806&22.28&14 \\ 
2017001509&17357&CANDELS\_13532&215.21909&53.07646&20.15&14 \\ 
2017001510&17426&CANDELS\_13536&215.16555&53.04128&23.89&9 \\ 
2017001557&17675&CANDELS\_13739&215.16329&53.04079&23.83&3 \\ 
2017001572&17769&CANDELS\_13794&215.17090&53.04545&23.37&14 \\ 
2017001611&18021&CANDELS\_13997&215.17558&53.05040&23.45&9 \\ 
2017001646&18160&CANDELS\_14117&215.19795&53.06685&22.80&3 \\ 
2017001662&18268&CANDELS\_14192&215.16401&53.04392&25.34&10 \\ 
2017001732&18721&CANDELS\_14530&215.17134&53.05038&23.75&9 \\ 
2017001767&18898&CANDELS\_14655&215.20187&53.07255&23.86&9 \\ 
2017001794&19074&CANDELS\_14792&215.16904&53.04958&23.07&3 \\ 
2017001892&19665&CANDELS\_15264&215.17038&53.05390&24.45&10 \\ 
2017001931&19887&CANDELS\_15422&215.18688&53.06652&24.68&7 \\ 
2017002023&20443&CANDELS\_15830&215.18318&53.06588&24.43&10 \\ 
2017002091&20710&CANDELS\_16123&215.18968&53.07089&23.82&3 \\ 
2017002126&20996&CANDELS\_16265&215.20199&53.08109&24.39&10 \\ 
2017002234&21660&CANDELS\_16741&215.18781&53.07402&25.84&7 \\ 
2017002252&21765&CANDELS\_16822&215.19353&53.07849&25.93&7 \\ 
2017002327&22206&CANDELS\_17185&215.17800&53.06928&25.57&15 \\ 
2017002353&22399&CANDELS\_17306&215.18060&53.07192&26.16&13 \\ 
2017002425&22739&CANDELS\_17592&215.18326&53.07354&21.94&3 \\ 
2017002427&22790&CANDELS\_17600&215.17681&53.07095&26.50&15 \\ 
2017002430&22670&CANDELS\_17626&215.18804&53.07685&22.22&3 \\ 
2017002448&22916&CANDELS\_17712&215.18118&53.07452&26.73&15 \\ 
2017002457&22949&CANDELS\_17749&215.17525&53.07038&25.34&7 \\ 
2017002509&23233&CANDELS\_17980&215.13011&53.03875&22.81&9 \\ 
2017002584&4636&&215.18088&53.07743&25.78&14 \\ 
2017002618&23948&CANDELS\_18471&215.17280&53.07237&25.06&7 \\ 
2017002660&24062&CANDELS\_18611&215.18630&53.08125&21.66&14 \\ 
2017002674&24140&CANDELS\_18673&215.12975&53.04238&23.74&9 \\ 
2017002690&24207&CANDELS\_18738&215.18396&53.08113&23.31&4 \\ 
2017002706&24326&CANDELS\_18796&215.13047&53.04326&23.17&5 \\ 
2017002750&24591&CANDELS\_18999&215.17993&53.07905&23.47&14 \\ 
2017002771&24667&CANDELS\_19089&215.12954&53.04476&25.16&14 \\ 
2017002819&25033&CANDELS\_19329&215.18480&53.08512&26.49&7 \\ 
2017002871&25295&CANDELS\_19554&215.11997&53.03995&23.34&5 \\ 
2017002894&25612&CANDELS\_19698&215.12740&53.04677&25.23&14 \\ 
2017002974&26006&CANDELS\_20091&215.12675&53.04836&25.76&10 \\ 
2017003005&26145&CANDELS\_20247&215.11919&53.04279&22.87&3 \\ 
2017003055&26525&CANDELS\_20508&215.13479&53.05592&25.48&11 \\ 
2017003129&27045&CANDELS\_20917&215.12488&53.05050&24.60&10 \\ 
2017003141&27211&CANDELS\_21030&215.13362&53.05766&26.20&8 \\ 
2017003184&27476&CANDELS\_21277&215.11766&53.04640&22.84&14 \\ 
2017003234&27940&CANDELS\_21601&215.12735&53.05622&26.08&15 \\ 
2017003248&28003&CANDELS\_21660&215.11162&53.04501&24.23&14 \\ 
2017003304&28499&CANDELS\_22045&215.12967&53.05985&25.76&15 \\ 
2017003354&28827&CANDELS\_22326&215.12899&53.06058&23.92&9 \\ 
2017003421&29354&CANDELS\_22743&215.10289&53.04432&24.77&10 \\ 
2017003456&29706&CANDELS\_23004&215.10828&53.04924&23.30&14 \\ 
2017003494&30061&CANDELS\_23247&215.13917&53.07257&24.63&10 \\ 
2017003752&32304&CANDELS\_24941&215.13703&53.07999&25.21&7 \\ 
2017003821&32814&CANDELS\_25359&215.13515&53.07708&20.07&14 \\ 
2017003837&33042&CANDELS\_25503&215.13138&53.07858&23.75&9 \\ 
2017003839&33064&CANDELS\_25508&215.13644&53.08219&23.56&9 \\ 
2017003845&33122&CANDELS\_25557&215.12855&53.07692&23.98&9 \\ 
2017003892&33521&CANDELS\_25869&215.14143&53.08796&25.58&10 \\ 
2017003921&33844&CANDELS\_26104&215.14127&53.08881&24.23&10 \\ 
2017003938&33985&CANDELS\_26195&215.13477&53.08507&25.29&15 \\ 
2017004017&34685&CANDELS\_26754&215.13103&53.08466&23.97&9 \\ 
2017004022&34779&CANDELS\_26787&215.13243&53.08656&26.73&8 \\ 
2017004056&35038&CANDELS\_27023&215.11766&53.07664&23.85&15 \\ 
2017004175&36047&CANDELS\_27771&215.12607&53.08714&25.52&15 \\ 
2017004179&36042&CANDELS\_27794&215.12221&53.08341&23.33&9 \\ 
2017004362&37322&CANDELS\_30633&215.12267&53.08998&26.05&10 \\ 
2017004369&37216&CANDELS\_30704&215.13293&53.09630&24.02&1 \\ 
2017004404&37134&CANDELS\_30950&215.13043&53.09370&24.13&11 \\ 
2017004681&&CANDELS\_34310&215.19041&53.03003&26.80&7 \\ 
2017004806&13349&CANDELS\_34999&215.18789&53.04089&26.61&7 \\ 
2017004859&&CANDELS\_35235&215.20805&53.05911&27.31&15 \\ 
2017004909&7431&&215.20401&53.06198&26.38&7 \\ 
2017004944&&CANDELS\_35736&215.16114&53.03504&26.61&10 \\ 
2017004946&&CANDELS\_35748&215.20580&53.06655&26.77&7 \\ 
2017004968&17079&CANDELS\_35850&215.17202&53.04464&26.95&14 \\ 
2017004975&17178&CANDELS\_35879&215.16121&53.03751&26.90&7 \\ 
2017004993&17531&CANDELS\_35972&215.17331&53.04756&26.59&10 \\ 
2017004999&17615&CANDELS\_35995&215.16489&53.04196&26.92&7 \\ 
2017005047&18637&CANDELS\_36251&215.19189&53.06502&26.87&7 \\ 
2017005135&391&&215.20653&53.08224&25.98&7 \\ 
2017005173&21430&CANDELS\_36862&215.18939&53.07425&26.61&13 \\ 
2017005194&&CANDELS\_36987&215.17356&53.06520&27.55&15 \\ 
2017005250&&CANDELS\_37236&215.13047&53.03949&26.54&7 \\ 
2017005261&&CANDELS\_37283&215.19005&53.08194&26.54&8 \\ 
2017005315&24465&CANDELS\_37565&215.17716&53.07751&26.86&15 \\ 
2017005393&&CANDELS\_37975&215.17852&53.08557&27.06&15 \\ 
2017005519&&CANDELS\_38798&215.11679&53.05632&27.29&8 \\ 
2017005560&&CANDELS\_39076&215.11014&53.05673&27.00&15 \\ 
2017005565&31321&CANDELS\_39114&215.10842&53.05625&26.01&7 \\ 
2017005605&&CANDELS\_39390&215.13443&53.07901&25.63&10 \\ 
2017005620&&CANDELS\_39455&215.12846&53.07586&27.38&10 \\ 
2017005637&&CANDELS\_39592&215.13967&53.08581&26.51&7 \\ 
2017005709&&CANDELS\_40074&215.13224&53.08912&26.82&14 \\ 
2017005743&&CANDELS\_40309&215.13563&53.09526&26.95&15 \\ 
2017005766&&CANDELS\_40514&215.12716&53.09258&26.84&15 \\ 
2017005963&1328&&215.20001&53.04060&26.83&8 \\ 
2017006007&3050&&215.18370&53.03436&25.37&10 \\ 
2017006046&4477&&215.19300&53.04543&24.72&7 \\ 
2017006097&6218&&215.16933&53.03410&25.71&14 \\ 
2017006211&9169&&215.16032&53.03679&25.07&10 \\ 
2017006241&17467&&215.20251&53.06783&25.67&7 \\ 
2017006677&7523&&215.13044&53.05056&25.05&7 \\ 
2017006681&7658&&215.18258&53.08643&23.56&14 \\ 
2017006812&11138&&215.11478&53.04961&24.04&7 \\ 
2017006936&1375&&215.10915&53.05556&23.72&9 \\ 
2017007560&&ACS\_1702\_845&215.18189&53.07964&-99.00&1 \\ 
2017007694&&ACS\_1703\_261&215.18887&53.02704&-99.00&14 \\ 
2017007757&&ACS\_1703\_25&215.19397&53.04585&-99.00&14 \\ 
2017007954&&HSC\_74648477224671846&215.21643&53.07336&-99.00&14 \\ 
2017008260&&HSC\_74648614663654360&215.11627&53.06350&-99.00&14 \\ 
2017008276&&HSC\_74648614663654223&215.11833&53.06098&-99.00&14 \\ 
2017008299&&HSC\_74648614663632280&215.12886&53.05515&-99.00&14 \\ 
2017008352&&HSC\_74648614663656333&215.11191&53.05978&-99.00&14 \\ 
2017008368&&HSC\_74648614663654165&215.10973&53.06078&-99.00&14 \\ 
2017008473&&HSC\_74648614663632253&215.11214&53.05156&-99.00&14 \\ 
2017008587&&HSC\_74648614663654861&215.12732&53.07347&-99.00&14 \\ 
2017008949&12014&CANDELS\_9368&215.19790&53.04241&24.92&1 \\ 
2017008950&34788&CANDELS\_26820&215.13865&53.08988&22.08&6 \\ 
2018000601&5429&CANDELS\_4315&215.11634&52.95565&23.10&14 \\ 
2018000680&6043&CANDELS\_4863&215.10894&52.95370&24.33&14 \\ 
2018000729&6552&CANDELS\_5169&215.11247&52.95863&24.01&15 \\ 
2018000800&7177&CANDELS\_5593&215.12066&52.96335&20.85&14 \\ 
2018000828&7319&CANDELS\_5748&215.10957&52.95993&25.24&7 \\ 
2018000856&7489&CANDELS\_5878&215.11684&52.96572&25.30&14 \\ 
2018000868&7544&CANDELS\_5942&215.11888&52.96733&24.70&7 \\ 
2018000975&8348&CANDELS\_6540&215.10768&52.96250&24.06&7 \\ 
2018000982&8397&CANDELS\_6572&215.11328&52.96729&25.09&7 \\ 
2018000983&8378&CANDELS\_6573&215.10595&52.96152&22.66&4 \\ 
2018000992&8462&CANDELS\_6621&215.12198&52.97297&24.59&7 \\ 
2018001021&8640&CANDELS\_6755&215.10658&52.96340&24.61&7 \\ 
2018001025&8708&CANDELS\_6792&215.11487&52.96870&23.33&14 \\ 
2018001077&9081&CANDELS\_7072&215.11676&52.97249&24.68&10 \\ 
2018001134&&CANDELS\_7387&215.09565&52.95929&23.72&5 \\ 
2018001187&9848&CANDELS\_7678&215.11584&52.97570&24.88&10 \\ 
2018001225&&CANDELS\_7876&215.09228&52.95771&22.81&14 \\ 
2018001228&10105&CANDELS\_7881&215.09292&52.96069&25.55&7 \\ 
2018001274&10414&CANDELS\_8089&215.10866&52.97328&25.96&15 \\ 
2018001283&&CANDELS\_8126&215.09164&52.95870&21.83&14 \\ 
2018001284&10403&CANDELS\_8127&215.13207&52.98939&23.75&9 \\ 
2018001286&10455&CANDELS\_8145&215.10025&52.96727&24.78&7 \\ 
2018001309&10612&CANDELS\_8288&215.12859&52.98797&24.66&7 \\ 
2018001327&10734&CANDELS\_8367&215.08604&52.95817&23.64&9 \\ 
2018001399&11224&CANDELS\_8722&215.12707&52.98964&26.08&15 \\ 
2018001489&11719&CANDELS\_9102&215.13063&52.99292&23.50&14 \\ 
2018001540&12010&CANDELS\_9335&215.12174&52.98837&24.69&10 \\ 
2018001591&12326&CANDELS\_9577&215.13953&53.00274&26.03&7 \\ 
2018001592&12288&CANDELS\_9579&215.13141&52.99574&21.93&3 \\ 
2018001623&&CANDELS\_9700&215.14123&53.00442&25.28&10 \\ 
2018001651&12479&CANDELS\_9835&215.13863&53.00104&22.59&1 \\ 
2018001677&12773&CANDELS\_9916&215.09802&52.97445&23.58&9 \\ 
2018001708&12936&CANDELS\_10079&215.09345&52.97258&24.85&15 \\ 
2018001765&13259&CANDELS\_10309&215.08836&52.97049&25.37&7 \\ 
2018001770&13258&CANDELS\_10321&215.12151&52.99386&25.10&14 \\ 
2018001829&13529&CANDELS\_10561&215.09124&52.97364&25.43&7 \\ 
2018001855&13690&CANDELS\_10688&215.11148&52.98832&24.93&14 \\ 
2018001899&13934&CANDELS\_10903&215.09014&52.97461&24.57&10 \\ 
2018001972&14413&CANDELS\_11247&215.11539&52.99381&24.24&14 \\ 
2018002014&14641&CANDELS\_11452&215.12099&52.99921&25.13&7 \\ 
2018002047&14824&CANDELS\_11571&215.11902&52.99730&22.36&14 \\ 
2018002253&16229&CANDELS\_12615&215.10393&52.99293&23.87&14 \\ 
2018002522&17899&CANDELS\_13895&215.10955&53.00426&26.72&10 \\ 
2018002541&18052&CANDELS\_13993&215.10436&53.00076&24.95&14 \\ 
2018002600&18540&CANDELS\_14389&215.05487&52.96811&25.15&15 \\ 
2018002614&18628&CANDELS\_14447&215.11109&53.00819&25.45&10 \\ 
2018002687&19085&CANDELS\_14790&215.09503&52.99883&25.61&15 \\ 
2018002737&19478&CANDELS\_15032&215.05324&52.97072&24.92&14 \\ 
2018002743&19399&CANDELS\_15058&215.09540&53.00010&24.83&10 \\ 
2018002754&19489&CANDELS\_15131&215.09568&52.99937&21.53&14 \\ 
2018002798&19778&CANDELS\_15342&215.05673&52.97404&23.86&9 \\ 
2018002816&12862&&215.05254&52.97227&24.23&14 \\ 
2018002841&20078&CANDELS\_15561&215.10558&53.01022&24.97&7 \\ 
2018002859&20114&CANDELS\_15611&215.09640&53.00169&20.53&14 \\ 
2018002896&20379&CANDELS\_15750&215.09920&53.00684&26.60&15 \\ 
2018002939&20557&CANDELS\_15935&215.09839&53.00583&22.25&14 \\ 
2018003059&21215&CANDELS\_16430&215.03957&52.96802&26.01&15 \\ 
2018003098&21425&CANDELS\_16594&215.04295&52.97123&25.25&1 \\ 
2018003115&21495&CANDELS\_16641&215.05782&52.98195&25.22&8 \\ 
2018003171&21857&CANDELS\_16887&215.04533&52.97458&26.00&7 \\ 
2018003236&22229&CANDELS\_17201&215.04757&52.97738&24.37&8 \\ 
2018003316&22767&CANDELS\_17582&215.04374&52.97723&26.00&8 \\ 
2018003382&23251&CANDELS\_17961&215.02882&52.96858&26.15&15 \\ 
2018003429&23594&CANDELS\_18225&215.02810&52.96944&26.15&8 \\ 
2018003491&23974&CANDELS\_18538&215.03181&52.97122&21.73&3 \\ 
2018003551&24349&CANDELS\_18830&215.03534&52.97719&24.61&10 \\ 
2018003587&24611&CANDELS\_19005&215.04082&52.98217&26.52&10 \\ 
2018003597&24648&CANDELS\_19058&215.03127&52.97498&24.20&11 \\ 
2018003618&24865&CANDELS\_19191&215.02506&52.97197&25.84&15 \\ 
2018003626&24941&CANDELS\_19229&215.03705&52.98066&25.42&7 \\ 
2018003650&25104&CANDELS\_19375&215.02833&52.97497&24.78&7 \\ 
2018003794&26013&CANDELS\_20119&215.03764&52.98481&24.04&10 \\ 
2018003809&26067&CANDELS\_20182&215.06352&53.00379&23.74&14 \\ 
2018003822&26175&CANDELS\_20266&215.06203&53.00201&22.14&9 \\ 
2018003832&26232&CANDELS\_20300&215.04108&52.98890&24.88&10 \\ 
2018003848&26395&CANDELS\_20415&215.03411&52.98440&25.42&1 \\ 
2018003875&26495&CANDELS\_20576&215.03104&52.98250&24.66&11 \\ 
2018003935&26981&CANDELS\_20864&215.05585&53.00109&23.44&9 \\ 
2018003945&27041&CANDELS\_20906&215.03463&52.98735&26.18&15 \\ 
2018004053&27662&CANDELS\_21436&215.05601&53.00453&24.32&7 \\ 
2018004077&27839&CANDELS\_21555&215.06716&53.01303&23.75&9 \\ 
2018004103&28058&CANDELS\_21702&215.04761&53.00048&26.06&15 \\ 
2018004144&28389&CANDELS\_21950&215.06650&53.01501&25.73&10 \\ 
2018004185&28835&CANDELS\_22263&215.06310&53.01323&22.70&9 \\ 
2018004263&29299&CANDELS\_22684&215.06376&53.01134&19.15&14 \\ 
2018004267&&EGSY-0120800269&215.05033&53.00747&25.15&1 \\ 
2018004291&29652&CANDELS\_22920&215.06348&53.01731&24.24&10 \\ 
2018004323&29773&CANDELS\_23077&215.06773&53.02019&21.60&14 \\ 
2018004326&29861&CANDELS\_23091&215.04127&53.00100&22.65&9 \\ 
2018004346&30070&CANDELS\_23232&215.05790&53.01570&26.43&11 \\ 
2018004358&30160&CANDELS\_23297&215.03908&53.00277&26.50&1 \\ 
2018004360&30091&CANDELS\_23319&215.05655&53.01351&22.69&9 \\ 
2018004466&31012&CANDELS\_23971&215.04206&53.00797&24.70&14 \\ 
2018004521&31751&CANDELS\_24533&215.04587&53.01385&24.66&10 \\ 
2018004536&31886&CANDELS\_24648&215.04269&53.01148&23.96&5 \\ 
2018005019&&CANDELS\_33437&215.10841&52.95627&27.46&15 \\ 
2018005281&&CANDELS\_34808&215.08332&52.96375&27.61&7 \\ 
2018005300&&CANDELS\_34901&215.09261&52.97199&27.09&14 \\ 
2018005303&&CANDELS\_34918&215.09535&52.97422&27.25&14 \\ 
2018005355&13957&CANDELS\_35143&215.11756&52.99405&26.56&10 \\ 
2018005401&&CANDELS\_35337&215.12278&53.00099&27.08&10 \\ 
2018005443&15960&CANDELS\_35590&215.11459&52.99968&26.36&7 \\ 
2018005482&&CANDELS\_35769&215.11806&53.00535&26.96&10 \\ 
2018005516&17188&CANDELS\_35883&215.12121&53.00946&27.05&7 \\ 
2018005533&&CANDELS\_35952&215.11926&53.00919&27.07&7 \\ 
2018005592&18534&CANDELS\_36216&215.05076&52.96527&26.52&15 \\ 
2018005605&&CANDELS\_36298&215.11205&53.00978&27.37&15 \\ 
2018005610&18966&CANDELS\_36333&215.05076&52.96705&27.08&14 \\ 
2018005777&&CANDELS\_37233&215.04423&52.97872&26.96&15 \\ 
2018005811&&CANDELS\_37423&215.05057&52.98621&27.06&15 \\ 
2018005873&&CANDELS\_37752&215.06111&52.99900&27.76&7 \\ 
2018005881&25410&CANDELS\_37785&215.02892&52.97694&26.62&15 \\ 
2018005922&&CANDELS\_37993&215.06505&53.00595&27.50&11 \\ 
2018005980&&CANDELS\_38365&215.05385&53.00437&27.01&15 \\ 
2018006055&&CANDELS\_38834&215.04166&53.00424&26.93&15 \\ 
2018006106&&CANDELS\_39189&215.04406&53.01202&27.18&15 \\ 
2018006588&1104&&215.12540&52.98686&24.59&10 \\ 
2018006747&4802&&215.09497&52.97771&24.86&10 \\ 
2018006862&7303&&215.10851&52.99440&26.68&14 \\ 
2018006899&8125&&215.10991&52.99822&26.46&8 \\ 
2018006971&10321&&215.09611&52.99569&28.09&7 \\ 
2018007017&12188&&215.11158&53.01196&24.72&7 \\ 
2018007552&624&&215.05951&53.01870&25.52&14 \\ 
2018007593&2010&&215.04457&53.01267&26.17&14 \\ 
2018007695&&EGSI-0280200176&215.11675&53.00489&26.51&1 \\ 
2018007732&&ACS\_1503\_1454&215.10031&52.97730&-99.00&14 \\ 
2018007939&&ACS\_1502\_662&215.05821&52.98033&-99.00&14 \\ 
2018008077&&HSC\_74648614663631762&215.04492&52.98621&-99.00&14 \\ 
2018008173&&HSC\_74648614663630710&215.06769&53.01546&-99.00&14 \\ 
2018008231&&HSC\_74648614663623810&215.09528&52.99373&-99.00&14 \\ 
2018008304&&HSC\_74648614663648010&215.09383&52.96641&-99.00&14 \\ 
2018008365&&HSC\_74648614663631629&215.11812&52.97311&-99.00&14 \\ 
2018008409&&HSC\_74648614663647880&215.08481&52.96490&-99.00&14 \\ 
2018008480&&HSC\_74648614663648805&215.05063&52.97972&-99.00&14 \\ 
2018008572&&HSC\_74648614663647745&215.11984&52.96212&-99.00&14 \\ 
2018009047&15073&CANDELS\_11822&215.08935&52.97784&23.42&3 \\ 
2018009063&19028&CANDELS\_14789&215.09468&52.99823&24.85&1 \\ 
2018009065&853&&215.10028&53.00453&19.55&6 \\ 
2019001016&9707&CANDELS\_7552&215.01113&52.90118&26.63&7 \\ 
2019001078&10225&CANDELS\_7898&215.01287&52.90144&20.83&14 \\ 
2019001086&10216&CANDELS\_7937&215.00599&52.89931&23.47&9 \\ 
2019001100&10289&CANDELS\_8003&215.01216&52.90449&25.21&7 \\ 
2019001121&10486&CANDELS\_8146&215.01178&52.90521&25.51&14 \\ 
2019001129&10523&CANDELS\_8174&215.01612&52.90789&24.87&15 \\ 
2019001139&10570&CANDELS\_8217&215.01827&52.90974&23.69&4 \\ 
2019001238&11357&CANDELS\_8792&215.01105&52.90806&25.18&7 \\ 
2019001297&11727&CANDELS\_9121&215.01749&52.91402&24.47&7 \\ 
2019001342&12085&CANDELS\_9366&215.01686&52.91470&24.44&7 \\ 
2019001360&12154&CANDELS\_9431&215.00996&52.91065&26.33&7 \\ 
2019001493&12964&CANDELS\_10089&215.01072&52.91415&25.13&7 \\ 
2019001519&13213&CANDELS\_10292&214.99868&52.90624&23.95&14 \\ 
2019001589&13715&CANDELS\_10652&214.99453&52.90572&24.96&10 \\ 
2019001610&13763&CANDELS\_10748&215.02889&52.93050&24.33&14 \\ 
2019001633&13882&CANDELS\_10830&215.00981&52.91759&25.51&7 \\ 
2019001658&14010&CANDELS\_10939&215.02698&52.93024&25.35&7 \\ 
2019001760&14721&CANDELS\_11483&214.98622&52.90422&25.60&7 \\ 
2019001767&14811&CANDELS\_11512&215.03112&52.93519&23.81&14 \\ 
2019001783&14944&CANDELS\_11634&214.98273&52.90227&25.09&10 \\ 
2019001790&15009&CANDELS\_11703&214.99941&52.91390&23.40&9 \\ 
2019001820&15173&CANDELS\_11841&215.02738&52.93485&25.20&15 \\ 
2019001835&15284&CANDELS\_11923&215.02036&52.92977&24.13&7 \\ 
2019001837&15310&CANDELS\_11938&214.98313&52.90356&23.67&4 \\ 
2019001842&15324&CANDELS\_11960&215.03370&52.94007&24.93&10 \\ 
2019001859&15448&CANDELS\_12031&215.03192&52.93749&23.04&14 \\ 
2019001889&15652&CANDELS\_12181&215.02245&52.93312&24.51&10 \\ 
2019001903&15775&CANDELS\_12276&214.98885&52.90999&25.33&7 \\ 
2019001924&15851&CANDELS\_12347&215.02975&52.93934&25.30&8 \\ 
2019001944&15981&CANDELS\_12437&214.98319&52.90697&25.27&8 \\ 
2019001958&16206&CANDELS\_12546&214.98356&52.90608&23.92&4 \\ 
2019001988&16427&CANDELS\_12736&215.03467&52.94425&23.36&9 \\ 
2019002003&16506&CANDELS\_12835&214.97900&52.90631&26.23&15 \\ 
2019002005&16526&CANDELS\_12843&214.99609&52.91844&26.00&7 \\ 
2019002017&16574&CANDELS\_12895&214.98640&52.91186&26.24&15 \\ 
2019002027&16648&CANDELS\_12944&214.99166&52.91585&26.04&7 \\ 
2019002046&16767&CANDELS\_13032&214.98935&52.91469&25.67&14 \\ 
2019002114&17147&CANDELS\_13340&215.02641&52.94209&24.53&14 \\ 
2019002164&17481&CANDELS\_13579&214.98885&52.91720&24.68&10 \\ 
2019002195&17772&CANDELS\_13818&214.98962&52.91837&23.02&14 \\ 
2019002320&18672&CANDELS\_14478&215.02787&52.94965&25.19&15 \\ 
2019002359&18973&CANDELS\_14715&214.98862&52.92292&24.24&7 \\ 
2019002512&20129&CANDELS\_15550&215.01711&52.94628&22.43&14 \\ 
2019002537&20297&CANDELS\_15695&215.00584&52.93937&22.85&12 \\ 
2019002539&20333&CANDELS\_15709&215.00012&52.93585&23.21&9 \\ 
2019002555&20435&CANDELS\_15788&214.99535&52.93348&24.81&15 \\ 
2019002564&20454&CANDELS\_15849&215.01037&52.94440&25.27&14 \\ 
2019002633&20997&CANDELS\_16255&215.01638&52.95086&26.23&7 \\ 
2019002715&21691&CANDELS\_16765&215.00789&52.94704&24.63&14 \\ 
2019002795&22245&CANDELS\_17203&214.99675&52.94180&25.51&7 \\ 
2019002810&22417&CANDELS\_17314&214.94789&52.90747&24.61&13 \\ 
2019002835&22575&CANDELS\_17441&214.99149&52.93891&23.93&4 \\ 
2019002874&22849&CANDELS\_17664&214.99598&52.94378&25.27&10 \\ 
2019002893&23068&CANDELS\_17827&214.99493&52.94338&23.63&4 \\ 
2019002908&23168&CANDELS\_17887&214.99006&52.94085&25.60&7 \\ 
2019002921&23219&CANDELS\_17951&215.00277&52.94971&24.41&7 \\ 
2019002934&23286&CANDELS\_18018&214.94782&52.91123&24.58&1 \\ 
2019002962&23491&CANDELS\_18168&214.99442&52.94478&23.83&4 \\ 
2019002986&23752&CANDELS\_18328&214.98969&52.94013&20.25&14 \\ 
2019002997&23789&CANDELS\_18424&214.94955&52.91391&23.32&9 \\ 
2019003013&24047&CANDELS\_18571&214.99606&52.94852&24.94&10 \\ 
2019003026&24162&CANDELS\_18691&214.99727&52.94761&22.50&1 \\ 
2019003077&24584&CANDELS\_19007&215.00230&52.95487&25.40&7 \\ 
2019003106&24770&CANDELS\_19156&214.93971&52.91106&24.70&7 \\ 
2019003128&24991&CANDELS\_19281&214.94474&52.91420&23.03&9 \\ 
2019003153&25125&CANDELS\_19421&214.94091&52.91349&25.18&10 \\ 
2019003269&25890&CANDELS\_20035&214.94499&52.91895&23.74&4 \\ 
2019003272&25934&CANDELS\_20047&214.95095&52.92395&25.48&1 \\ 
2019003338&26412&CANDELS\_20421&214.94794&52.92369&26.36&15 \\ 
2019003432&27092&CANDELS\_20984&214.95002&52.92703&23.81&12 \\ 
2019003485&27559&CANDELS\_21324&214.94137&52.92277&24.19&8 \\ 
2019003492&27624&CANDELS\_21385&214.94317&52.92388&23.26&9 \\ 
2019003550&28007&CANDELS\_21770&214.93257&52.91836&23.08&4 \\ 
2019003553&28192&CANDELS\_21804&214.92599&52.91497&25.74&14 \\ 
2019003586&28431&CANDELS\_21998&214.94538&52.92957&25.25&10 \\ 
2019003589&28472&CANDELS\_22022&214.93509&52.92244&26.04&7 \\ 
2019003604&28545&CANDELS\_22088&214.93336&52.92148&25.62&11 \\ 
2019003612&28622&CANDELS\_22133&214.92050&52.91269&26.48&15 \\ 
2019003638&28894&CANDELS\_22356&214.93952&52.92661&23.23&9 \\ 
2019003639&28901&CANDELS\_22369&214.95779&52.93986&24.76&11 \\ 
2019003659&29106&CANDELS\_22532&214.92005&52.91359&22.79&9 \\ 
2019003661&29149&CANDELS\_22543&214.92572&52.91861&25.61&1 \\ 
2019003679&29259&CANDELS\_22649&214.92856&52.92065&23.92&4 \\ 
2019003686&29332&CANDELS\_22690&214.92350&52.91773&26.81&15 \\ 
2019003713&29510&CANDELS\_22815&214.93019&52.92275&24.74&15 \\ 
2019003778&30072&CANDELS\_23228&214.93533&52.92806&23.69&9 \\ 
2019003782&30125&CANDELS\_23253&214.92096&52.91524&20.92&14 \\ 
2019003905&31270&CANDELS\_24140&214.95867&52.95032&25.44&10 \\ 
2019003957&31697&CANDELS\_24479&214.96220&52.95417&23.14&14 \\ 
2019003961&31786&CANDELS\_24512&214.95047&52.94598&23.32&14 \\ 
2019003982&31994&CANDELS\_24685&214.95043&52.94666&22.68&14 \\ 
2019003998&32094&CANDELS\_24766&214.95236&52.94900&25.68&15 \\ 
2019004071&&EGSV-9472256523&214.94675&52.94786&25.79&15 \\ 
2019004083&33012&CANDELS\_25443&214.94207&52.94505&25.34&10 \\ 
2019004116&33445&CANDELS\_25755&214.95313&52.95377&22.58&3 \\ 
2019004122&33462&CANDELS\_25800&214.94769&52.95063&23.72&9 \\ 
2019004151&33863&CANDELS\_26048&214.94211&52.94642&22.29&1 \\ 
2019004163&33975&CANDELS\_26163&214.95032&52.95490&25.74&15 \\ 
2019004168&34033&CANDELS\_26215&214.94837&52.95385&26.30&10 \\ 
2019004170&34004&CANDELS\_26229&214.93695&52.94547&24.51&10 \\ 
2019004184&34263&CANDELS\_26403&214.94204&52.95023&25.36&2 \\ 
2019004193&34340&CANDELS\_26462&214.93337&52.94438&25.09&14 \\ 
2019004214&34678&CANDELS\_26717&214.95478&52.96089&26.00&14 \\ 
2019004221&34768&CANDELS\_26777&214.93472&52.94709&26.51&1 \\ 
2019004638&&CANDELS\_34380&215.00097&52.89777&26.88&15 \\ 
2019004808&&CANDELS\_35338&214.99137&52.90835&26.33&10 \\ 
2019004830&15394&CANDELS\_35456&214.97912&52.90172&26.81&7 \\ 
2019004885&16701&CANDELS\_35764&215.01942&52.93570&26.75&14 \\ 
2019004948&&CANDELS\_36117&214.98682&52.91832&27.18&15 \\ 
2019005035&20053&CANDELS\_36580&215.00130&52.93656&27.37&15 \\ 
2019005072&21051&CANDELS\_36767&215.01279&52.94857&26.42&15 \\ 
2019005172&23283&CANDELS\_37296&214.94276&52.90776&26.67&15 \\ 
2019005192&&CANDELS\_37426&214.99373&52.94607&27.75&15 \\ 
2019005235&24876&CANDELS\_37663&215.00016&52.95442&26.84&10 \\ 
2019005384&28188&CANDELS\_38428&214.93858&52.92393&26.96&10 \\ 
2019005437&&CANDELS\_38771&214.92658&52.92160&26.76&15 \\ 
2019005451&&CANDELS\_38837&214.92867&52.92436&26.50&15 \\ 
2019005480&&CANDELS\_39108&214.94777&52.94277&27.33&11 \\ 
2019005551&&CANDELS\_39851&214.95092&52.95704&27.35&7 \\ 
2019005568&35381&CANDELS\_40061&214.95048&52.96063&26.76&10 \\ 
2019005961&3257&&215.01100&52.91333&nan&14 \\ 
2019005987&4251&&215.02697&52.92782&26.68&15 \\ 
2019006104&7609&&214.99013&52.91184&26.20&8 \\ 
2019006117&8251&&214.98966&52.91355&25.74&7 \\ 
2019006263&780&&215.00202&52.93950&26.55&15 \\ 
2019006289&1621&&215.01731&52.95289&25.70&7 \\ 
2019006295&1917&&215.01200&52.95001&26.48&7 \\ 
2019006308&&EGSY-9597563148&214.99893&52.94205&25.05&1 \\ 
2019006311&2624&&214.99036&52.93698&26.27&10 \\ 
2019006420&8907&&214.93748&52.91833&26.18&1 \\ 
2019006473&11387&&214.94367&52.93041&26.60&10 \\ 
2019006600&5476&&214.95316&52.95851&25.76&11 \\ 
2019006881&&ACS\_1402\_279&215.00134&52.91840&-99.00&14 \\ 
2019007187&&HSC\_74648610368662436&214.99666&52.89793&-99.00&14 \\ 
2019007246&&HSC\_74648614663645239&214.95108&52.92017&-99.00&14 \\ 
2019007453&&HSC\_74648614663631488&214.94585&52.95893&-99.00&14 \\ 
2019007481&&HSC\_74648614663646776&214.95525&52.94700&-99.00&14 \\ 
2019007500&&HSC\_74648614663631381&214.99394&52.94691&-99.00&14 \\ 
2019007515&&HSC\_74648614663631445&214.94348&52.95416&-99.00&14 \\ 
2019007879&&HSC\_74648614663630947&215.01059&52.90736&-99.00&14 \\ 
2020000264&4127&CANDELS\_3322&214.90618&52.80213&24.28&14 \\ 
2020000290&4353&CANDELS\_3523&214.90590&52.80304&25.19&14 \\ 
2020000301&4486&CANDELS\_3606&214.91460&52.80964&24.71&10 \\ 
2020000340&4821&CANDELS\_3876&214.91344&52.81041&24.10&14 \\ 
2020000376&5121&CANDELS\_4097&214.90845&52.80793&24.28&10 \\ 
2020000398&5326&CANDELS\_4214&214.91855&52.81529&23.87&14 \\ 
2020000466&5964&CANDELS\_4667&214.92392&52.82193&23.34&14 \\ 
2020000574&6851&CANDELS\_5402&214.89590&52.80655&24.47&7 \\ 
2020000586&7015&CANDELS\_5464&214.89778&52.80768&23.60&9 \\ 
2020000671&7575&CANDELS\_6026&214.90642&52.81688&24.38&7 \\ 
2020000684&7751&CANDELS\_6083&214.90416&52.81594&23.50&14 \\ 
2020000703&7941&CANDELS\_6216&214.92991&52.83548&25.27&15 \\ 
2020000727&8139&CANDELS\_6365&214.90863&52.82107&24.64&7 \\ 
2020000736&8251&CANDELS\_6416&214.90995&52.82164&24.90&10 \\ 
2020000745&8284&CANDELS\_6461&214.90041&52.81513&24.07&7 \\ 
2020000854&9126&CANDELS\_7112&214.92581&52.83809&26.45&14 \\ 
2020000866&9190&CANDELS\_7158&214.88121&52.80665&26.46&7 \\ 
2020000894&9376&CANDELS\_7306&214.88795&52.81103&23.22&9 \\ 
2020000901&9399&CANDELS\_7332&214.88402&52.80953&25.53&7 \\ 
2020000955&9806&CANDELS\_7649&214.89406&52.81846&24.54&14 \\ 
2020000963&9877&CANDELS\_7674&214.89817&52.82184&26.67&10 \\ 
2020000967&9899&CANDELS\_7693&214.93647&52.84910&26.05&15 \\ 
2020000992&10046&CANDELS\_7828&214.93663&52.84967&25.21&14 \\ 
2020000996&10065&CANDELS\_7852&214.93671&52.84726&20.48&14 \\ 
2020001030&10355&CANDELS\_8032&214.88570&52.81492&25.37&15 \\ 
2020001055&10445&CANDELS\_8134&214.93902&52.85325&24.48&7 \\ 
2020001076&10597&CANDELS\_8232&214.92550&52.84431&25.48&7 \\ 
2020001078&10599&CANDELS\_8245&214.92242&52.84234&26.07&7 \\ 
2020001081&10608&CANDELS\_8255&214.94005&52.85375&21.74&14 \\ 
2020001083&10636&CANDELS\_8277&214.88521&52.81574&25.00&8 \\ 
2020001085&10627&CANDELS\_8293&214.92900&52.84705&25.44&7 \\ 
2020001110&10832&CANDELS\_8410&214.89215&52.82079&23.45&5 \\ 
2020001111&11028&CANDELS\_8436&214.90020&52.82514&20.03&14 \\ 
2020001229&11880&CANDELS\_9140&214.91954&52.84197&22.54&9 \\ 
2020001235&11823&CANDELS\_9170&214.91533&52.84155&24.69&7 \\ 
2020001349&3071&&214.89311&52.82795&24.38&14 \\ 
2020001408&12913&CANDELS\_10031&214.90730&52.84087&26.19&15 \\ 
2020001494&13428&CANDELS\_10463&214.90382&52.84006&23.50&14 \\ 
2020001495&13456&CANDELS\_10464&214.90121&52.83813&24.88&1 \\ 
2020001666&14347&CANDELS\_11166&214.91141&52.84873&24.65&10 \\ 
2020001726&14786&CANDELS\_11521&214.90792&52.84876&25.48&7 \\ 
2020001756&14943&CANDELS\_11659&214.89958&52.84156&22.49&14 \\ 
2020001970&16391&CANDELS\_12727&214.89785&52.84737&24.27&7 \\ 
2020001975&16425&CANDELS\_12766&214.89791&52.84841&26.34&8 \\ 
2020001992&16473&CANDELS\_12831&214.90902&52.85655&25.54&7 \\ 
2020002024&16673&CANDELS\_12981&214.84728&52.81277&23.20&14 \\ 
2020002063&16986&CANDELS\_13206&214.89831&52.84901&23.19&9 \\ 
2020002081&17134&CANDELS\_13292&214.89398&52.84743&24.42&14 \\ 
2020002129&17494&CANDELS\_13577&214.85106&52.81954&26.36&15 \\ 
2020002200&17865&CANDELS\_13899&214.84875&52.81915&24.52&13 \\ 
2020002269&18376&CANDELS\_14249&214.85278&52.82424&25.87&15 \\ 
2020002337&18777&CANDELS\_14559&214.90190&52.85987&23.09&12 \\ 
2020002375&19002&CANDELS\_14728&214.84603&52.82203&26.00&10 \\ 
2020002397&19168&CANDELS\_14902&214.85573&52.82822&19.75&14 \\ 
2020002486&19760&CANDELS\_15288&214.83553&52.81766&25.87&10 \\ 
2020002545&20162&CANDELS\_15598&214.84048&52.82241&24.63&15 \\ 
2020002567&20291&CANDELS\_15703&214.85106&52.83076&25.36&10 \\ 
2020002632&20764&CANDELS\_16087&214.84036&52.82496&24.94&2 \\ 
2020002742&&CANDELS\_16722&214.82968&52.82077&26.26&1 \\ 
2020002767&21788&CANDELS\_16848&214.82374&52.81697&24.73&15 \\ 
2020002787&&CANDELS\_16921&214.84869&52.83524&24.95&10 \\ 
2020002811&22058&CANDELS\_17081&214.86216&52.84541&25.05&7 \\ 
2020002835&22188&CANDELS\_17217&214.83921&52.82932&24.52&10 \\ 
2020002912&22722&CANDELS\_17570&214.82579&52.82217&24.19&14 \\ 
2020002967&23072&CANDELS\_17820&214.82251&52.82148&26.48&15 \\ 
2020003005&23456&CANDELS\_18122&214.84141&52.83587&23.50&4 \\ 
2020003014&23537&CANDELS\_18175&214.82447&52.82470&26.37&7 \\ 
2020003073&4788&&214.82474&52.82624&26.40&15 \\ 
2020003119&24174&CANDELS\_18676&214.85836&52.85129&25.77&7 \\ 
2020003139&24280&CANDELS\_18761&214.82912&52.83016&23.19&12 \\ 
2020003216&24882&CANDELS\_19181&214.82634&52.82932&23.10&9 \\ 
2020003242&25055&CANDELS\_19318&214.86368&52.85790&24.88&2 \\ 
2020003275&25323&CANDELS\_19527&214.82892&52.83324&23.01&14 \\ 
2020003304&&CANDELS\_19696&214.85580&52.85467&26.57&1 \\ 
2020003317&25568&CANDELS\_19750&214.86480&52.86051&24.39&7 \\ 
2020003326&25620&CANDELS\_19797&214.86580&52.86187&24.66&2 \\ 
2020003342&25712&CANDELS\_19874&214.85573&52.85531&24.98&15 \\ 
2020003389&26056&CANDELS\_20126&214.85109&52.85332&25.27&8 \\ 
2020003424&26351&CANDELS\_20341&214.85979&52.86064&25.40&1 \\ 
2020003493&26910&CANDELS\_20709&214.86120&52.86349&24.49&15 \\ 
2020003494&26784&CANDELS\_20716&214.84681&52.85249&22.88&14 \\ 
2020003509&26921&CANDELS\_20814&214.84454&52.85206&25.72&8 \\ 
2020003601&27524&CANDELS\_21289&214.84969&52.85818&26.82&14 \\ 
2020003634&27761&CANDELS\_21483&214.85007&52.85953&26.60&10 \\ 
2020003688&28080&CANDELS\_21789&214.83903&52.85208&24.53&14 \\ 
2020003758&28638&CANDELS\_22148&214.85941&52.86936&26.44&10 \\ 
2020004509&4957&CANDELS\_32999&214.90940&52.80833&27.03&15 \\ 
2020004552&&CANDELS\_33274&214.90884&52.81202&27.83&11 \\ 
2020004658&8388&CANDELS\_33869&214.92684&52.83535&27.02&15 \\ 
2020004678&&CANDELS\_33959&214.89193&52.81208&26.62&15 \\ 
2020004685&&CANDELS\_34012&214.93598&52.84458&26.70&15 \\ 
2020004717&&CANDELS\_34194&214.88553&52.81237&26.81&14 \\ 
2020004733&9942&CANDELS\_34239&214.89603&52.82059&27.19&7 \\ 
2020005006&&CANDELS\_35682&214.89419&52.84524&28.19&15 \\ 
2020005049&17448&CANDELS\_35958&214.90758&52.85956&26.76&7 \\ 
2020005064&&CANDELS\_36008&214.85294&52.82163&27.16&10 \\ 
2020005156&&CANDELS\_36403&214.83686&52.81659&27.88&8 \\ 
2020005205&20084&CANDELS\_36584&214.84431&52.82521&27.34&10 \\ 
2020005210&&CANDELS\_36616&214.85073&52.83030&26.81&7 \\ 
2020005238&20899&CANDELS\_36743&214.83421&52.82115&25.92&8 \\ 
2020005308&22379&CANDELS\_37081&214.83596&52.82824&26.96&10 \\ 
2020005349&23400&CANDELS\_37322&214.82429&52.82403&27.40&10 \\ 
2020005589&28773&CANDELS\_38547&214.84744&52.86137&27.48&11 \\ 
2020005626&&CANDELS\_38826&214.84756&52.86657&27.01&14 \\ 
2020005887&378&&214.92397&52.82007&25.23&7 \\ 
2020005892&506&&214.92413&52.82087&26.62&14 \\ 
2020005924&528&&214.89707&52.80556&24.07&10 \\ 
2020005975&49&&214.92987&52.83612&26.53&15 \\ 
2020006047&306&&214.91616&52.83641&25.93&10 \\ 
2020006050&10422&&214.89867&52.82476&26.06&7 \\ 
2020006214&4593&&214.92083&52.85574&28.34&7 \\ 
2020006236&5514&&214.91328&52.85144&25.52&7 \\ 
2020006251&5644&&214.91462&52.85287&26.59&10 \\ 
2020006321&7191&&214.85300&52.81313&26.86&14 \\ 
2020006322&7327&&214.90664&52.85172&25.92&15 \\ 
2020006346&7735&&214.90879&52.85451&25.85&7 \\ 
2020006366&8295&&214.90177&52.85127&27.53&7 \\ 
2020006373&8479&&214.89410&52.84651&26.67&7 \\ 
2020006380&8616&&214.84714&52.81363&27.45&10 \\ 
2020006401&9168&&214.91024&52.86017&27.24&7 \\ 
2020006406&9348&&214.84848&52.81680&26.19&8 \\ 
2020006425&9986&&214.90144&52.85646&26.97&8 \\ 
2020006426&9977&&214.89880&52.85256&22.19&9 \\ 
2020006552&420&&214.83365&52.81872&24.93&14 \\ 
2020006562&863&&214.84595&52.82899&26.22&8 \\ 
2020006632&2789&&214.82195&52.81799&26.06&11 \\ 
2020006650&3220&&214.83147&52.82589&26.70&11 \\ 
2020006651&3245&&214.84277&52.83413&25.97&13 \\ 
2020006796&8410&&214.84423&52.85055&25.42&14 \\ 
2020006823&9164&&214.86509&52.86767&26.11&7 \\ 
2020006853&9948&&214.85259&52.86122&27.08&10 \\ 
2020006916&11245&&214.84032&52.85624&26.91&14 \\ 
2020006946&11837&&214.84284&52.86004&25.47&8 \\ 
2020007227&&ACS\_1102\_1059&214.84457&52.84969&-99.00&14 \\ 
2020007493&&HSC\_74648610368664788&214.92114&52.81793&-99.00&14 \\ 
2020007536&&HSC\_74648747807617567&214.85666&52.86289&-99.00&14 \\ 
2020007552&&HSC\_74648747807619072&214.86249&52.86550&-99.00&14 \\ 
2020007667&&HSC\_74648747807611792&214.85358&52.82574&-99.00&14 \\ 
2020008022&&HSC\_74648610368685448&214.90131&52.84273&-99.00&14 \\ 
2020008149&&HSC\_74648610368663247&214.90807&52.80704&-99.00&14 \\ 
2020008189&&HSC\_74648610368659465&214.89207&52.84618&-99.00&14 \\ 
2020008402&&HSC\_74648610368683829&214.92040&52.81744&-99.00&14 \\ 
2020008613&&HSC\_74648610368683750&214.90105&52.81586&-99.00&14 \\ 
2020008652&11766&CANDELS\_9156&214.92126&52.84573&23.46&3 \\ 
2021000689&8236&CANDELS\_6432&214.83977&52.77277&26.79&14 \\ 
2021000811&9326&CANDELS\_7248&214.83388&52.77329&25.41&15 \\ 
2021000906&10251&CANDELS\_7967&214.83054&52.77495&24.88&8 \\ 
2021000937&10448&CANDELS\_8109&214.83662&52.78037&25.22&7 \\ 
2021000962&10561&CANDELS\_8219&214.84112&52.78407&24.49&8 \\ 
2021000982&10739&CANDELS\_8351&214.84200&52.78562&26.74&15 \\ 
2021001024&11004&CANDELS\_8571&214.83812&52.78359&23.87&14 \\ 
2021001025&11054&CANDELS\_8589&214.82053&52.77167&26.28&10 \\ 
2021001033&11080&CANDELS\_8610&214.81939&52.77097&26.39&8 \\ 
2021001080&11637&CANDELS\_8953&214.82482&52.77650&25.27&7 \\ 
2021001089&11644&CANDELS\_9035&214.82875&52.77971&24.79&11 \\ 
2021001097&11682&CANDELS\_9087&214.81732&52.77181&25.53&7 \\ 
2021001177&12389&CANDELS\_9606&214.81366&52.77126&23.34&14 \\ 
2021001180&12440&CANDELS\_9624&214.82292&52.77836&24.86&10 \\ 
2021001181&2966&&214.83160&52.78505&26.57&15 \\ 
2021001189&12482&CANDELS\_9691&214.83990&52.79117&25.78&13 \\ 
2021001241&&CANDELS\_9994&214.81079&52.77156&24.99&15 \\ 
2021001255&12917&CANDELS\_10037&214.82578&52.78103&22.63&14 \\ 
2021001275&13046&CANDELS\_10151&214.83335&52.78816&24.93&7 \\ 
2021001286&13149&CANDELS\_10227&214.82179&52.78113&27.00&14 \\ 
2021001303&13290&CANDELS\_10355&214.83417&52.78959&24.25&15 \\ 
2021001372&13799&CANDELS\_10737&214.83035&52.78939&24.54&15 \\ 
2021001439&14205&CANDELS\_11089&214.82680&52.78872&24.76&10 \\ 
2021001505&14695&CANDELS\_11472&214.81980&52.78567&24.10&13 \\ 
2021001508&14722&CANDELS\_11498&214.82333&52.78841&24.94&14 \\ 
2021001551&15231&CANDELS\_11746&214.81843&52.78617&24.35&15 \\ 
2021001636&15644&CANDELS\_12191&214.81176&52.78371&25.70&7 \\ 
2021001695&15993&CANDELS\_12454&214.81747&52.78906&25.07&7 \\ 
2021001734&16285&CANDELS\_12638&214.81432&52.78774&23.58&9 \\ 
2021001796&16608&CANDELS\_12906&214.81326&52.78889&25.56&15 \\ 
2021001815&16690&CANDELS\_12983&214.80664&52.78378&23.63&5 \\ 
2021001905&17344&CANDELS\_13465&214.78339&52.77068&26.38&11 \\ 
2021001921&17453&CANDELS\_13555&214.83831&52.81032&26.23&14 \\ 
2021002003&17941&CANDELS\_13920&214.84016&52.81085&21.56&14 \\ 
2021002071&18387&CANDELS\_14260&214.83905&52.81452&25.94&7 \\ 
2021002161&19037&CANDELS\_14760&214.82671&52.80841&26.14&10 \\ 
2021002245&&CANDELS\_15190&214.77775&52.77601&25.41&14 \\ 
2021002283&&CANDELS\_15386&214.77690&52.77636&26.17&7 \\ 
2021002334&&CANDELS\_15714&214.83628&52.82041&26.10&10 \\ 
2021002388&20790&CANDELS\_16080&214.76476&52.77023&23.07&14 \\ 
2021002390&20764&CANDELS\_16087&214.84036&52.82496&24.94&2 \\ 
2021002434&21174&CANDELS\_16382&214.83723&52.82435&26.19&7 \\ 
2021002438&21208&CANDELS\_16406&214.76551&52.77331&25.28&8 \\ 
2021002442&21241&CANDELS\_16443&214.82116&52.81247&23.07&3 \\ 
2021002450&21250&CANDELS\_16471&214.81551&52.80894&24.08&7 \\ 
2021002479&21547&CANDELS\_16663&214.77520&52.78134&24.98&15 \\ 
2021002493&21599&CANDELS\_16714&214.81667&52.81138&25.40&7 \\ 
2021002496&&CANDELS\_16722&214.82968&52.82077&26.26&1 \\ 
2021002513&&CANDELS\_16810&214.83160&52.82206&25.13&13 \\ 
2021002542&21906&CANDELS\_16931&214.77426&52.78218&24.99&7 \\ 
2021002582&22216&CANDELS\_17160&214.77013&52.78020&24.49&7 \\ 
2021002586&22263&CANDELS\_17186&214.83887&52.82962&25.34&15 \\ 
2021002587&22251&CANDELS\_17188&214.83489&52.82248&20.74&14 \\ 
2021002608&22384&CANDELS\_17290&214.80998&52.80973&25.22&1 \\ 
2021002691&23026&CANDELS\_17774&214.76016&52.77662&25.19&10 \\ 
2021002716&23164&CANDELS\_17924&214.81215&52.81439&24.87&10 \\ 
2021002727&23250&CANDELS\_17966&214.81132&52.81356&22.70&3 \\ 
2021002728&23263&CANDELS\_17968&214.80777&52.81121&23.37&14 \\ 
2021002746&23388&CANDELS\_18072&214.80445&52.80984&25.89&15 \\ 
2021002750&23449&CANDELS\_18116&214.81306&52.81618&25.56&15 \\ 
2021002751&23538&CANDELS\_18124&214.76865&52.78414&24.87&15 \\ 
2021002800&23737&CANDELS\_18336&214.74921&52.77184&25.52&15 \\ 
2021002825&23901&CANDELS\_18462&214.81979&52.82217&23.39&9 \\ 
2021002866&24308&CANDELS\_18781&214.75897&52.78093&25.57&11 \\ 
2021002921&24696&CANDELS\_19098&214.81494&52.82227&25.30&7 \\ 
2021002988&25232&CANDELS\_19478&214.75672&52.78251&25.25&15 \\ 
2021003024&25530&CANDELS\_19728&214.81372&52.82276&21.63&14 \\ 
2021003099&26098&CANDELS\_20171&214.80970&52.82424&25.49&15 \\ 
2021003100&26101&CANDELS\_20175&214.81570&52.82758&24.02&10 \\ 
2021003218&9167&&214.80806&52.82688&26.01&7 \\ 
2021003234&&CANDELS\_21039&214.77484&52.80357&25.16&10 \\ 
2021003310&&CANDELS\_21496&214.77322&52.80483&25.89&14 \\ 
2021003368&28219&CANDELS\_21820&214.80359&52.82809&26.36&7 \\ 
2021003375&28253&CANDELS\_21872&214.80547&52.82938&24.93&14 \\ 
2021003589&30217&CANDELS\_23328&214.77715&52.81412&19.90&14 \\ 
2021003600&30398&CANDELS\_23493&214.76208&52.80709&24.96&7 \\ 
2021003624&30611&CANDELS\_23625&214.76735&52.81161&25.28&7 \\ 
2021003738&31672&CANDELS\_24433&214.76814&52.81655&26.66&1 \\ 
2021003768&31867&CANDELS\_24632&214.75103&52.80447&23.47&4 \\ 
2021003776&31977&CANDELS\_24681&214.75397&52.80699&23.95&9 \\ 
2021003795&32279&CANDELS\_24818&214.78279&52.82770&22.93&14 \\ 
2021003796&32182&CANDELS\_24819&214.75205&52.80579&23.56&9 \\ 
2021003831&32398&CANDELS\_24999&214.78127&52.82857&26.45&15 \\ 
2021003841&32495&CANDELS\_25089&214.78035&52.82827&25.09&7 \\ 
2021003846&32570&CANDELS\_25139&214.75596&52.81076&23.10&14 \\ 
2021003856&32713&CANDELS\_25236&214.77201&52.82324&26.41&15 \\ 
2021003858&&CANDELS\_25242&214.77920&52.80478&19.69&14 \\ 
2021003890&33070&CANDELS\_25488&214.75685&52.81337&24.59&14 \\ 
2021003895&33143&CANDELS\_25548&214.74775&52.80757&26.09&14 \\ 
2021003912&33324&CANDELS\_25691&214.77394&52.82703&25.80&7 \\ 
2021003916&33372&CANDELS\_25737&214.77734&52.82937&23.81&14 \\ 
2021003939&33633&CANDELS\_25930&214.77830&52.82922&22.52&14 \\ 
2021003963&33944&CANDELS\_26150&214.76554&52.82352&26.61&7 \\ 
2021004010&34442&CANDELS\_26522&214.74890&52.81270&23.64&9 \\ 
2021004049&35001&CANDELS\_26993&214.76233&52.82509&24.57&10 \\ 
2021004074&35417&CANDELS\_27210&214.75989&52.82469&24.75&15 \\ 
2021004084&35554&CANDELS\_27405&214.76435&52.82908&26.53&15 \\ 
2021004115&36009&CANDELS\_27718&214.75069&52.82102&26.02&15 \\ 
2021004127&27430&CANDELS\_27811&214.76907&52.80324&12.43&14 \\ 
2021004155&37261&CANDELS\_31109&214.74742&52.82368&25.18&7 \\ 
2021004157&36951&CANDELS\_31161&214.75287&52.82652&25.63&8 \\ 
2021004434&9054&CANDELS\_34032&214.83468&52.77287&27.03&14 \\ 
2021004464&&CANDELS\_34243&214.83586&52.77784&28.08&8 \\ 
2021004572&12686&CANDELS\_34854&214.80974&52.77048&26.77&15 \\ 
2021004696&&CANDELS\_35472&214.80588&52.77891&27.17&15 \\ 
2021004724&16342&CANDELS\_35694&214.80991&52.78545&27.15&8 \\ 
2021004801&18199&CANDELS\_36146&214.83197&52.80875&26.57&15 \\ 
2021004904&20917&CANDELS\_36741&214.82545&52.81498&26.77&7 \\ 
2021004912&21115&CANDELS\_36776&214.81809&52.81052&26.59&14 \\ 
2021004976&22460&CANDELS\_37098&214.75534&52.77106&26.62&7 \\ 
2021004991&22970&CANDELS\_37209&214.76103&52.77724&27.19&15 \\ 
2021005013&23390&CANDELS\_37318&214.82347&52.82339&26.82&10 \\ 
2021005023&23512&CANDELS\_37349&214.76203&52.78010&27.48&10 \\ 
2021005041&&CANDELS\_37453&214.76320&52.78273&25.80&7 \\ 
2021005068&24614&CANDELS\_37597&214.75790&52.78128&26.58&15 \\ 
2021005092&&CANDELS\_37761&214.82078&52.82886&27.43&15 \\ 
2021005114&26077&CANDELS\_37943&214.80482&52.82075&27.07&15 \\ 
2021005147&27030&CANDELS\_38160&214.80679&52.82569&26.70&15 \\ 
2021005216&&CANDELS\_38631&214.78487&52.81839&27.09&15 \\ 
2021005225&29423&CANDELS\_38693&214.77981&52.81587&27.02&10 \\ 
2021005292&31382&CANDELS\_39130&214.75800&52.80814&26.73&7 \\ 
2021005308&&CANDELS\_39247&214.77299&52.82082&26.87&7 \\ 
2021005361&33755&CANDELS\_39699&214.77070&52.82648&26.72&15 \\ 
2021005720&2487&&214.81466&52.77158&26.72&15 \\ 
2021005961&10343&&214.78465&52.77331&23.67&9 \\ 
2021005966&10511&&214.78050&52.77190&25.19&7 \\ 
2021005988&11120&&214.77928&52.77274&23.59&9 \\ 
2021006040&12258&&214.82408&52.80852&23.95&14 \\ 
2021006059&12800&&214.78518&52.78238&27.43&7 \\ 
2021006083&741&&214.77243&52.77605&26.08&7 \\ 
2021006096&1174&&214.83366&52.82106&26.25&14 \\ 
2021006106&1400&&214.78170&52.78465&24.36&14 \\ 
2021006134&1940&&214.81916&52.81329&26.63&7 \\ 
2021006182&3477&&214.75434&52.77191&26.13&10 \\ 
2021006214&&EGSZ-9135048459&214.80625&52.81275&26.55&1 \\ 
2021006242&5514&&214.82564&52.82886&25.90&7 \\ 
2021006317&8202&&214.78125&52.80525&25.47&7 \\ 
2021006361&9719&&214.77662&52.80637&28.22&7 \\ 
2021006394&10573&&214.77208&52.80571&25.94&10 \\ 
2021006452&12446&&214.76502&52.80632&25.82&14 \\ 
2021006471&12799&&214.76357&52.80658&25.12&7 \\ 
2021006475&41&&214.76644&52.80886&24.88&7 \\ 
2021006497&655&&214.76024&52.80647&25.82&15 \\ 
2021006634&&EGSV-9161749471&214.81737&52.82975&24.96&1 \\ 
2021006718&&ACS\_1101\_1100&214.74951&52.82377&-99.00&15 \\ 
2021006728&&ACS\_1002\_1073&214.77023&52.80958&-99.00&15 \\ 
2021006828&&ACS\_1102\_683&214.81465&52.80803&-99.00&15 \\ 
2021007799&&HSC\_74648747807636177&214.81639&52.78902&-99.00&15 \\ 
2021007883&&HSC\_74648747807636318&214.75957&52.80330&-99.00&15 \\ 
2021008021&19743&CANDELS\_15327&214.82924&52.80843&20.57&1 \\ 
2021008037&25372&CANDELS\_19611&214.75012&52.77807&22.96&6 \\ 
 \end{longtable}
}

